Spot and Facula Activity Variations of the Eccentric Detached Eclipsing Binary KIC 8098300 Based on the Time-series Orbital Solutions

The LAMOST spectra and $\it{Kepler}$ light curves are combined to investigate the detached eclipsing binary KIC 8098300, which shows the O'Connell effect caused by spot/facula modulation. The radial velocity (RV) measurements are derived by using the tomographic spectra disentangling technology. The mass ratio $q = K_1/K_2 = 0.812 \pm 0.007$, and the orbital semi-major axis $a\mathrm{\sin}i = 14.984 \pm 0.048\ R_\odot$ are obtained by fitting the RV curves. We optimize the binary model concerning the spot/facula activity with the code PHOEBE and obtain precise parameters of the orbit including the eccentricity $e=0.0217 \pm 0.0008$, the inclination $i=87.71\pm 0.04^\circ$, and the angle of periastron $\omega=284.1\pm 0.5^\circ$. The masses and radii of the primary and secondary star are determined as $M_1=1.3467 \pm 0.0001\ M_\odot$, $R_1=1.569 \pm 0.003\ R_\odot$, and $M_2=1.0940 \pm 0.0001\ M_\odot$, $R_2=1.078 \pm 0.002\ R_\odot$, respectively. The ratio of temperatures of the two component stars is $r_{teff}=0.924 \pm 0.001$. We also obtain the periastron precession speed of $0.000024\pm 0.000001\ \mathrm{d}\ cycle^{-1}$. The residuals of out-of-eclipse are analyzed using the Auto-Correlation Function (ACF) and the Discrete Fourier Transform (DFT). The spot/facula activity is relatively weaker, but the lifetime is longer than that of most single main sequence stars in the same temperature range. The average rotation period of the spots $P_{rot}=4.32\ d$ is slightly longer than the orbital period, which may be caused by either the migration of spots/faculae along the longitude or the latitudinal differential rotation. The activity may be spot-dominated for the secondary star and facula-dominated for the primary star.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

